Ballooning Multi-Armed Bandits

In this paper, we introduce Ballooning Multi-Armed Bandits (BL-MAB), a novel extension of the classical stochastic MAB model. In the BL-MAB model, the set of available arms grows (or balloons) over time. In contrast to the classical MAB setting where the regret is computed with respect to the best arm overall, the regret in a BL-MAB setting is computed with respect to the best available arm at each time. We first observe that the existing stochastic MAB algorithms result in linear regret for the BL-MAB model. We prove that, if the best arm is equally likely to arrive at any time instant, a sub-linear regret cannot be achieved. Next, we show that if the best arm is more likely to arrive in the early rounds, one can achieve sub-linear regret. Our proposed algorithm determines (1) the fraction of the time horizon for which the newly arriving arms should be explored and (2) the sequence of arm pulls in the exploitation phase from among the explored arms. Making reasonable assumptions on the arrival distribution of the best arm in terms of the thinness of the distribution's tail, we prove that the proposed algorithm achieves sub-linear instance-independent regret. We further quantify explicit dependence of regret on the arrival distribution parameters. We reinforce our theoretical findings with extensive simulation results. We conclude by showing that our algorithm would achieve sub-linear regret even if (a) the distributional parameters are not exactly known, but are obtained using a reasonable learning mechanism or (b) the best arm is not more likely to arrive early, but a large fraction of arms is likely to arrive relatively early.

==> BL-prelims.tex <==
\section{Preliminaries}
%\textcolor{red}{Need to see that each notation is defined before using it}
\label{sec:BL-prelims}
    We now present some  essential concepts which will be useful for our analysis in the remainder of the chapter.
\subsection{Lambert $W$ Function}
%We first present its definition.
\begin{definition}
%[{Lambert $W$ function}]
    \label{def:lambert}
       For any $x>-e^{-1}$, the Lambert $W$ function, $W(x)$, is defined as the solution to the equation $w e^{w} = x$, i.e., $W(x)e^{W(x)} = x$.
    \end{definition}
%In the non-negative domain, 
Lambert $W$ function satisfies the following properties\cite{hoorfar2008inequalities}.   
     \begin{lemma}
   \label{prop:zero}
   The Lambert $W$ function can be equivalently written as the inverse of the function $f(x) := xe^{x}$, i.e., $W(xe^{x}) =x$.  
   \end{lemma}
\begin{proof}
	The forward direction is straightforward. As $W(\cdot)$ is one to one function in the non-negative domain,  we have $W(W(x)e^{W(x)}) =  W(x)$. Let $y = W(x)$ then we have $W(ye^{y}) = y$. To show that $W(xe^{x}) = x$ implies $W(z)e^{W(z)} = z$, observe that $W(W(z_0)e^{W(z_0)}) = W(z_0)$.  We get the required result by taking the inverse. 
\end{proof}
     \begin{lemma}
   \label{prop:two}
   For any $x \in [0, \infty)$, the Lambert $W$ function is unique, non-negative, and strictly increasing. 
   \end{lemma}
\begin{proof}
	Observe that $W(0) = 0$. Note that  $ f(x) =xe^{x}$ is continuous, one to one and strictly increasing. Hence, its inverse, $W(\cdot)$,  is also increasing.  
\end{proof}

   \begin{lemma}
   \label{prop:one}
   For any $x \geq e$, we have  $\log(x)/2 < W(x) \leq  \log(x) $. 
   \end{lemma}
\begin{proof}
	By definition, the Lambert $W$ function satisfies $W(x)e^{W(x)} = x$. It is easy to see that $W(e) = 1$. Further we have,
	\begin{align*}
	1 & = \frac{dW(x)}{dx} \cdot e^{W(x)} + \frac{dW(x)}{dx} \cdot e^{W(x)} W(x)  \\
	& = \frac{dW(x)}{dx} (x + e^{W(x)}) \\ 
	\implies  \frac{dW(x)}{dx} &= \frac{1}{x + e^{W(x)}}
	\end{align*}
	Let $f(x) = \log(x) - W(x)$. We have that $f(e) = 0$. We have that $\frac{df(x)}{dx} = \frac{1}{x} - \frac{1}{x + e^{W(x)}} = \frac{e^{W(x)}}{x(x + e^{W(x)})} = \frac{1}{x(1+W(x))} > 0$. Hence we have that $f(\cdot)$ is increasing i.e. $f(x) >0$ for all $x > e$. This shows that $W(x) \leq \log(x)$.
	
	Now, let $g(x)=\frac{\log(x)}{2}-W(x)$. Here, we have $g(e)<0$, and $\frac{dg(x)}{dx} = \frac{1}{2x}- \frac{1}{x + e^{W(x)}} = \frac{e^{W(x)}-e^{\log(x)}}{2x(x + e^{W(x)})} \leq 0$ (since $W(x)\leq \log(x)$ for $x\geq e$).
	So, $g(x)<0$ for all $x \geq e$, implying that $\frac{\log(x)}{2}<W(x)$.
	%
	This completes the proof. 
	%
\end{proof}

It can be noted that it is easy to numerically approximate $W(x)$ for a given $x$, using Newton-Raphson's  or Halley's method. Moreover, there exist efficient numerical methods for evaluating it to arbitrary precision \cite{Corless1996}.

   
   %   \subsection{Hoeffding-Azuma inequality}
%   \label{ssec:hoeffding}
   
   \subsection{The \Moss Algorithm}
   We use  \Moss (Minimax Optimal Strategy in the Stochastic case)~\cite{audibert2010regret} as a black box learning algorithm. For a fixed number of $k$ arms, the   \Moss algorithm pulls an arm $i_t$ at time $t$ where $$i_t \in  \arg \max_{i \in K} \Bigg [\hat{q}_{i, N_{i,t}} + \sqrt{\frac{\max(\log(\frac{T}{k \cdot N_{i,t}}), 0)}{N_{i,t}}}\Bigg ].$$
    Here, $K = \{1,2, \cdots, k \}$ denotes the set of arms and  $N_{i,t}$ is the number of times arm $i$ was pulled before (and excluding) round $t$ and $\hat{q}_{i,N_{i,t}}$ are the empirical estimates of the arm $i$  from $N_{i,t}$ samples. 
    %
    %The corner cases are handled as follows. 
    %
    Each arm is pulled once in the beginning, and ties are broken arbitrarily.   
   The following result gives an upper bound on the expected regret of \Moss which is optimal up to a constant factor (it achieves the lower bound on regret given by \cite{auer1995gambling}). Throughout the chapter, we use the notation \Moss(K) to denote that the \Moss algorithm is run with set of arms $K$. 
   %\textcolor{red}{As per usage in Algorithm 1, $K$ looks like a set. But here it is mentioned as number of arms.}
   %\textcolor{red}{$K$ is sometimes used as a set and sometimes as a number.}\textcolor{brown}{the last sentence could be in model that K indicates set of arms as well as number of arms in K interchangbly}
   %\textcolor{red}{But this can be abit confusing, because we are considering that arms arrive at each time, so $K$ is then also the time when the $K^{\text{th}}$ arm arrives. So $K$ would then be the index of the $K^{\text{th}}$ arm as well as the set of arms $\{1,\ldots,K\}$. This is ok if it's a standard practice, else some reviewers may find it mind-boggling.}
   
   \begin{restatable}{theorem}{mossRegret}[\cite{audibert2010regret}]
   \label{thm:moss_regret}
   For any time horizon $T\geq 1$, the expected regret of \Moss is given by $  \mathcal{R}_{\moss}(T) \leq 6 \sqrt{k T }$.
   \end{restatable}
   
%  \textcolor{red}{$K$ is used for fixed number of arms and $K(t)$ is used for denoting set of arms. Hope this is ok?}\textcolor{brown}{depends upon the reviewer...some reviewers are fine..but would suggest better to use different notation if possible. }
   


==> Ballooning.tex <==
\chapter{Ballooning Multi Armed Bandits}
\label{chap:Ballooning}
\input{Ballooning/BL-abstract.tex}
\input{Ballooning/BL-intro.tex}
\input{Ballooning/BL-model.tex}
\input{Ballooning/BL-lowerBound.tex}
\input{Ballooning/BL-prelim.tex}
%\input{proposed.tex}
\input{Ballooning/BL-results.tex}
%\input{Applications.tex}
\input{Ballooning/BL-simulation.tex}
\input{Ballooning/BL-RelWork.tex}
\input{Ballooning/BL-discussion.tex}
\newpage
\input{Ballooning/BL-appendix.tex}


